Generating Images with 3D Annotations Using Diffusion Models

Diffusion models have emerged as a powerful generative method, capable of producing stunning photo-realistic images from natural language descriptions. However, these models lack explicit control over the 3D structure in the generated images. Consequently, this hinders our ability to obtain detailed 3D annotations for the generated images or to craft instances with specific poses and distances. In this paper, we propose 3D Diffusion Style Transfer (3D-DST), which incorporates 3D geometry control into diffusion models. Our method exploits ControlNet, which extends diffusion models by using visual prompts in addition to text prompts. We generate images of the 3D objects taken from 3D shape repositories (e.g., ShapeNet and Objaverse), render them from a variety of poses and viewing directions, compute the edge maps of the rendered images, and use these edge maps as visual prompts to generate realistic images. With explicit 3D geometry control, we can easily change the 3D structures of the objects in the generated images and obtain ground-truth 3D annotations automatically. This allows us to improve a wide range of vision tasks, e.g., classification and 3D pose estimation, in both in-distribution (ID) and out-of-distribution (OOD) settings. We demonstrate the effectiveness of our method through extensive experiments on ImageNet-100/200, ImageNet-R, PASCAL3D+, ObjectNet3D, and OOD-CV. The results show that our method significantly outperforms existing methods, e.g., 3.8 percentage points on ImageNet-100 using DeiT-B.

==> figures/supp_LLM_simple_prompt.tex <==
\begin{figure}[!t]
    \centering
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.24\textwidth]{DST/5_0}
    \includegraphics[width=0.24\textwidth]{DST/9_1}
    \includegraphics[width=0.24\textwidth]{DST/14_0}
    \includegraphics[width=0.24\textwidth]{DST/15_0}
    \includegraphics[width=0.24\textwidth]{DST/23_0}
    \includegraphics[width=0.24\textwidth]{DST/24_1}
    \includegraphics[width=0.24\textwidth]{DST/48_0}
    \includegraphics[width=0.24\textwidth]{DST/50_0}
    \caption{3D-DST data with diverse prompts from LLM.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.24\textwidth]{DST_simple/5_0}
    \includegraphics[width=0.24\textwidth]{DST_simple/9_0}
    \includegraphics[width=0.24\textwidth]{DST_simple/14_0}
    \includegraphics[width=0.24\textwidth]{DST_simple/15_0}
    \includegraphics[width=0.24\textwidth]{DST_simple/23_0}
    \includegraphics[width=0.24\textwidth]{DST_simple/24_0}
    \includegraphics[width=0.24\textwidth]{DST_simple/48_0}
    \includegraphics[width=0.24\textwidth]{DST_simple/50_0}
    \caption{3D-DST data with simple prompts.}
    \end{subfigure}
    \caption{Qualitative comparison between 3D-DST data generated with diverse prompts with LLM and simple prompts crafted by hand.}
    \label{fig:comparison}
\end{figure}

==> figures/supp_more_images.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/1_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/2_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/3_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/4_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/5_0}
    \end{subfigure} \\
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/6_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/7_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/8_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/9_1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/10_0}
    \end{subfigure} \\
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/11_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/12_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/13_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/14_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/15_0}
    \end{subfigure} \\
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/16_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/17_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/18_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/19_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/20_0}
    \end{subfigure} \\
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/21_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/22_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/23_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/24_1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/25_0}
    \end{subfigure} \\
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/26_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/27_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/28_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/29_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/30_0}
    \end{subfigure} \\
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/31_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/32_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/33_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/34_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/35_0}
    \end{subfigure} \\
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/36_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/37_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/38_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/39_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/40_0}
    \end{subfigure} \\
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/41_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/42_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/43_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/44_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/45_0}
    \end{subfigure} \\
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/46_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/47_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/48_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/49_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{}
    \centering
    \includegraphics[width=0.16\textwidth]{DST/50_0}
    \end{subfigure}
    \caption{Samples images from our 3D-DST dataset.}
    \label{fig:sample_50}
\end{figure}



==> sections/4_method_3d_aware_pretraining.tex <==
\subsection{3D-Aware Pre-Training}

Pretrained feature extractors derived from a classification model trained on the ImageNet dataset have been widely adopted in various downstream applications, consistently showing high efficacy. \citep{he2023is} also demonstrated that pretraining vision models on synthetic data generated with text-to-image diffusion models can also lead to promising results on multiple downstream tasks. However, existing pre-trained vision models mostly rely on 2D-based supervision, such as image classification or masked image modeling, due to the limited supervision signals available. In this work, we explore the benefits of 3D-based supervision given our \OursCls dataset with rich 3D annotations.

\paragraph{Classification-based pre-training on ImageNet.} We represent the ImageNet dataset as $\{(I_i, y_i)\}_{i=1}^N$ where each image $I_i$ is paired with a class label $y_i \in \mathbb{Y} = \{y_1, \dots, y_{C}\}$. During pre-training, the vision feature extractor $\Phi$ is concatenated with a $C$-class classifier head, producing a logit value $s_i$ for each class $y_i$. Then the whole model is updated with a cross-entropy loss given by
\begin{align*}
    \mathcal{L}_\text{cls} = \sum_{i=1}^N - \log \frac{\exp (s_{y_i})}{\sum_{j=1}^C \exp(s_j)}.
\end{align*}

\paragraph{3D-aware pre-training on \OursCls.} In \OursCls dataset, each image $I_i$ is paired with rich 2D and 3D annotations, including class label $y_i$, 3D viewpoint specified by azimuth $a_i$, elevation $e_i$, and in-plane rotation $\theta_i$ w.r.t. the world coordinate system, distance from the camera to the object $d_i$, as well as 3D shape of the object given by a reference to a known 3D model $m_i$. Thus we represent \OursCls dataset as $\{(I_i, y_i, a_i, e_i, \theta_i, d_i, m_i)\}_{i=1}^M$.

To allow the pre-trained vision model to reason with a 3D perspective, a straightforward idea is to add 3D viewpoint estimation supervision to the existing classification loss. Following \citep{tulsiani2015viewpoints}, we formulate the viewpoint estimation problem as a bin classification for each of $a_i$, $e_i$, and $\theta_i$. This leads us to a viewpoint estimation loss given by
\begin{align}
    \mathcal{L}_\text{viewpoint} = \sum_{i=1}^N - \log \frac{\exp(s_{a, \hat{a}_i})}{\sum_{j=1}^{C_v} \exp(s_{a, j})} - \log \frac{\exp(s_{e, \hat{e}_i})}{\sum_{j=1}^{C_v} \exp(s_{e, j})} - \log \frac{\exp(s_{\theta, \hat{\theta}_i})}{\sum_{j=1}^{C_v} \exp(s_{\theta, j})}
\end{align}
where $\hat{a}_i$, $\hat{e}_i$, $\hat{\theta}_i$ are the ground-truth bin indices, $s_{a, i}$, $s_{e, i}$, $s_{\theta, i}$ are the logit values for azimuth/elevation/in-plane rotation bin $i$, and $C_v$ is the number of bins for each viewpoint angle. Lastly, a multi-task loss $\mathcal{L} = \mathcal{L}_\text{cls} + \mathcal{L}_\text{viewpoint}$ is used during the pre-training stage.

\paragraph{Relaxing the multi-task trade-off.} Although the viewpoint estimation loss can encourage the classification model to learn and benefit from 3D-discriminative features, it inevitably introduces a trade-off between class discrimination and 3D awareness. Therefore, we propose a 3D aware loss that can effectively alleviate the trade-off by learning from a weaker but highly effective 3D supervision.

xxx.

In Section~\ref{sec4_img_cls} and Section~\ref{sec4_3d_pose} we demonstrate that vision models pretrained with our 3D-awareness loss achieve improved performance on downstream tasks, including image classification and 3D pose estimation on both independently and identically distributed and out-of-distribution data.

==> tables/ablation.tex <==
\begin{table}
\centering
{\renewcommand\arraystretch{1.1}
\setlength{\tabcolsep}{2.8mm}{
\begin{tabular}{cccllcllcccccc}
    \toprule
    \multirow{2.5}{*}{{No.}} & \multirow{1.5}{*}{{3D-DST}} & \multirow{2.5}{*}{{LLM}}  & \multicolumn{2}{c}{In-distribution (ID)} && \multicolumn{2}{c}{Out-of-distribution (OOD)} \\
    \cmidrule{4-5} \cmidrule{7-8}
    & (pre-train) & & ResNet & ViT && ResNet & ViT \\
    \midrule


    1 &&  &   86.60 {\scriptsize\textcolor{white}{($\uparrow$0.00)}} & 84.72 {\scriptsize\textcolor{white}{($\uparrow$0.00)}} && 50.60 {\scriptsize\textcolor{white}{($\uparrow$0.00)}} & 42.81 {\scriptsize\textcolor{white}{($\uparrow$0.00)}} \\
    2 &\checkmark&  &   88.96   {\scriptsize\textcolor{ablation_green}{($\uparrow$2.36)}} & 88.72 {\scriptsize\textcolor{ablation_green}{($\uparrow$4.00)}}  && 53.97 {\scriptsize\textcolor{ablation_green}{($\uparrow$3.37)}} & 45.30 {\scriptsize\textcolor{ablation_green}{($\uparrow$2.49)}} \\
    3 &\checkmark& \checkmark &   \textbf{89.28} {\scriptsize\textcolor{ablation_green}{($\uparrow$2.68)}} & \textbf{89.36} {\scriptsize\textcolor{ablation_green}{($\uparrow$4.64)}} && \textbf{54.14} {\scriptsize\textcolor{ablation_green}{($\uparrow$3.54)}} & \textbf{48.52} {\scriptsize\textcolor{ablation_green}{($\uparrow$5.71)}} \\

    \\[-14pt]
    \bottomrule
\end{tabular}}}
\vspace{-0.2cm}
\caption{Ablation Study (\%) in the ID and OOD settings. Numbers in brackets show rise/fall compared to the baseline. For ID, we use a $50$-class subset of ImageNet. For OOD, we use ImageNet-R. Line~1 shows the baseline results without pre-training. Line~2 shows the results using the model pre-trained on our 3D-DST data. Line~3 shows the results of applying our LLM prompts based on Line 2.}
\label{tab:ablation}
\end{table}


% \begin{table}
% \centering
% {\renewcommand\arraystretch{1.0}
% \setlength{\tabcolsep}{2.8mm}{
% \begin{tabular}{ccclllclllcccccc}
%     \toprule
%     \multirow{2.5}{*}{{Row}} & \multirow{1.5}{*}{{3D-DST}} & \multirow{2.5}{*}{{LLM}}  & \multicolumn{2}{c}{In-distribution (ID)} && \multicolumn{2}{c}{Out-of-distribution (OOD)} \\
%     \cmidrule{4-5} \cmidrule{7-8}
%     & (Pre-train) & & ResNet & ViT && ResNet & ViT \\
%     \midrule
%     1 &&  &   - {\scriptsize\textcolor{white}{($\uparrow$0.00)}} & - {\scriptsize\textcolor{white}{($\uparrow$0.00)}} && - {\scriptsize\textcolor{white}{($\uparrow$0.00)}} & - {\scriptsize\textcolor{white}{($\uparrow$-)}} \\
%     2 &\checkmark&  &   -   {\scriptsize\textcolor{ablation_green}{($\uparrow$-)}} & - {\scriptsize\textcolor{ablation_green}{($\uparrow$-)}}  && - {\scriptsize\textcolor{ablation_green}{($\uparrow$-)}} & - {\scriptsize\textcolor{ablation_green}{($\uparrow$-)}} \\
%     3 &\checkmark& \checkmark &   \textbf{-} {\scriptsize\textcolor{ablation_green}{($\uparrow$-)}} & \textbf{-} {\scriptsize\textcolor{ablation_green}{($\uparrow$-)}} && \textbf{-} {\scriptsize\textcolor{ablation_green}{($\uparrow$-)}} & \textbf{-} {\scriptsize\textcolor{ablation_green}{($\uparrow$-)}} \\

%     \\[-14pt]
%     \bottomrule
% \end{tabular}}}
% \vspace{-0.2cm}
% \caption{Ablation Study (\%) on ImageNet-$100$ (ID) and ImageNet-R (OOD). Numbers in brackets show rise/fall compared to the baseline. Line~1 shows the baseline results without pre-training. Line~2 shows the results using the model pre-trained on our 3D-DST data. Line~3 shows the results of applying our LLM prompts based on Line 2.}
% \label{tab:ablation}
% \end{table}

==> tables/compare_datagen_main.tex <==
\begin{table}
\centering
{\renewcommand\arraystretch{1.1}
\setlength{\tabcolsep}{1mm}{
\begin{tabular}{llllllll}
    \toprule
    \multirow{2.5}{*}{{Methods}}  & \multicolumn{2}{c}{Classification} && \multicolumn{2}{c}{Pose Estimation} \\
    \cmidrule{2-3}
    \cmidrule{5-6}
     & ACC@ID & ACC@OOD && ACC@$\pi/6$ & MedErr \\
    \midrule
    Baseline & 84.56 {\scriptsize\textcolor{white}{($\uparrow$0.00)}} & 49.61 {\scriptsize\textcolor{white}{$\uparrow$0.00}} && 70.6 {\scriptsize\textcolor{white}{$\uparrow$0.0}} & 23.6 {\scriptsize\textcolor{white}{$\uparrow$0.0}} \\
    \emph{\ \ w /} Text2Img \citeyearpar{he2023is} & 84.80 {\scriptsize\textcolor{ablation_green}{($\uparrow$0.24)}} & 50.83 {\scriptsize\textcolor{ablation_green}{($\uparrow$1.22)}} \\
    \emph{\ \ w /} ImageNet edges & 85.20 {\scriptsize\textcolor{ablation_green}{($\uparrow$0.64)}} & 48.69 {\scriptsize\textcolor{ablation_red}{($\downarrow$0.92)}} \\
    \emph{\ \ w /} Rendering + BG2D & 84.96 {\scriptsize\textcolor{ablation_green}{($\uparrow$0.40)}} & 50.92 {\scriptsize\textcolor{ablation_green}{($\uparrow$1.31)}} && 75.9 {\scriptsize\textcolor{ablation_green}{($\uparrow$5.3)}} & 17.1 {\scriptsize\textcolor{ablation_green}{($\downarrow$6.5)}} \\
    \emph{\ \ w /} Rendering + BG3D & 87.50 {\scriptsize\textcolor{ablation_green}{($\uparrow$2.94)}} & 54.81 {\scriptsize\textcolor{ablation_green}{($\uparrow$5.20)}} && 76.2 {\scriptsize\textcolor{ablation_green}{($\uparrow$5.6)}} & 16.4 {\scriptsize\textcolor{ablation_green}{($\downarrow$7.2)}} \\
    \cellcolor{mygray-bg}{\emph{\ \ w /} \OursCls (ours)} & \cellcolor{mygray-bg}{\textbf{88.96} {\scriptsize\textcolor{ablation_green}{($\uparrow$4.40)}}} & \cellcolor{mygray-bg}{\textbf{56.65} {\scriptsize\textcolor{ablation_green}{($\uparrow$7.04)}}} & \cellcolor{mygray-bg}{} & \cellcolor{mygray-bg}{\textbf{79.2} {\scriptsize\textcolor{ablation_green}{($\uparrow$8.6)}}} & \cellcolor{mygray-bg}{\textbf{14.1} {\scriptsize\textcolor{ablation_green}{($\downarrow$9.5)}}} \\
    \\[-14pt]
    \bottomrule
\end{tabular}}}
\caption{\textbf{Ablation study of data generation methods on image classification and pose estimation.} We report top-1 accuracy~(\%) on ImageNet-$100$ (ID) and ImageNet-R (OOD) using DeiT-S. For pose estimation we use NeMo \cite{Wang2021NeMo} and report the pose accuracy at $\pi/6$ and median error. We compare the performances when models are trained purely on the target dataset or pre-trained on synthetic dataset with different data generation methods. Please refer to Section~\ref{sec:supp_ablation_datagen} for specifics of each data generation approach.}
\label{tab:exp-ablation-datagen}
\end{table}


==> tables/supp_ablation_datagen_pose.tex <==
\begin{table}
\centering
{\renewcommand\arraystretch{1.1}
\setlength{\tabcolsep}{1mm}{
\revision{
\begin{tabular}{llllllll}
    \toprule
    Methods & ACC@$\pi/6$ & ACC@$\pi/18$ & MedErr \\
    \midrule
    NeMo~\citep{Wang2021NeMo} & 70.6 {\scriptsize\textcolor{white}{$\uparrow$0.0}} & 46.5 {\scriptsize\textcolor{white}{$\uparrow$0.0}} & 23.6 {\scriptsize\textcolor{white}{$\uparrow$0.0}} \\
    \emph{\ \ w /} Rendering + BG2D & 75.9 {\scriptsize\textcolor{ablation_green}{($\uparrow$5.3)}} & 47.8 {\scriptsize\textcolor{ablation_green}{($\uparrow$1.3)}} & 17.1 {\scriptsize\textcolor{ablation_green}{($\downarrow$6.5)}} \\
    \emph{\ \ w /} Rendering + BG3D & 76.2 {\scriptsize\textcolor{ablation_green}{($\uparrow$5.6)}} & 49.3 {\scriptsize\textcolor{ablation_green}{($\uparrow$2.8)}} & 16.4 {\scriptsize\textcolor{ablation_green}{($\downarrow$7.2)}} \\
    \cellcolor{mygray-bg}{\emph{\ \ w /} 3D-DST (ours)} & \cellcolor{mygray-bg}{\textbf{79.2} {\scriptsize\textcolor{ablation_green}{($\uparrow$8.6)}}} & \cellcolor{mygray-bg}{\textbf{52.0} {\scriptsize\textcolor{ablation_green}{($\uparrow$5.5)}}} & \cellcolor{mygray-bg}{\textbf{14.1} {\scriptsize\textcolor{ablation_green}{($\downarrow$9.5)}}} \\
    \\[-14pt]
    \bottomrule
\end{tabular}}}}
\caption{\revision{\textbf{Ablation study of data generation methods on pose estimation.} We adopt the state-of-the-art 3D pose estimation model \citep{Wang2021NeMo} as the baseline model and compare the performance with different data generation methods. Please refer to Section~\ref{sec:supp_ablation_datagen} for specifics of each data generation approach.}}
\label{tab:exp-ablation-datagen-pose}
\end{table}

==> tables/supp_class_iid_50.tex <==
\begin{table}
\begin{center}
\begin{tabular}{ c|l } 
\hline
synset &class name \\
\hline
\underline{n01443537} &goldfish, Carassius auratus \\
n01514668 &cock \\
\underline{n01855672} &goose \\
\underline{n02007558} &flamingo \\
\underline{n02129165} &lion, king of beasts, Panthera leo \\
\underline{n02129604} &tiger, Panthera tigris \\
n02342885 &hamster \\
\underline{n02391049} &zebra \\
\underline{n02510455} &giant panda, panda, panda bear, coon bear, Ailuropoda melanoleuca \\
n02676566 &acoustic guitar \\
n02690373 &airliner \\
\underline{n02701002} &ambulance \\
n02747177 &ashcan, trash can, garbage can, wastebin, ash bin, ash-bin, ashbin, dustbin, trash barrel, trash bin \\
\underline{n02808440} &bathtub, bathing tub, bath, tub \\
n02814533 &beach wagon, station wagon, wagon, estate car, beach waggon, station waggon, waggon \\
\underline{n02843684} &birdhouse \\
n02930766 &cab, hack, taxi, taxicab \\
\underline{n02992529} &cellular telephone, cellular phone, cellphone, cell, mobile phone \\
n03063599 &coffee mug \\
n03085013 &computer keyboard, keypad \\
n03095699 &container ship, containership, container vessel \\
n03187595 &dial telephone, dial phone \\
n03201208 &dining table, board \\
\underline{n03452741} &grand piano, grand \\
n03642806 &laptop, laptop computer \\
n03658185 &letter opener, paper knife, paperknife \\
n03709823 &mailbag, postbag \\
\underline{n03710193} &mailbox, letter box \\
n03761084 &microwave, microwave oven \\
n03792782 &mountain bike, all-terrain bike, off-roader \\
n03891251 &park bench \\
n03938244 &pillow \\
n03977966 &police van, police wagon, paddy wagon, patrol wagon, wagon, black Maria \\
n03983396 &pop bottle, soda bottle \\
n03991062 &pot, flowerpot \\
n04004767 &printer \\
n04074963 &remote control, remote \\
\underline{n04146614} &school bus \\
n04263257 &soup bowl \\
n04330267 &stove \\
n04344873 &studio couch, day bed \\
n04380533 &table lamp \\
n04487081 &trolleybus, trolley coach, trackless trolley \\
\underline{n04552348} &warplane, military plane \\
n04554684 &washer, automatic washer, washing machine \\
n04557648 &water bottle \\
\underline{n07720875} &bell pepper \\
\underline{n07745940} &strawberry \\
\underline{n07753275} &pineapple, ananas \\
\underline{n07753592} &banana \\
\hline
\end{tabular}
\vspace{0.3cm}
\caption{The related ImageNet synsets and class names of the 50 classes used in 3D-DST classification. The 19 synsets with underlines are the classes overlapping with ImageNet-R that are used in OOD experiments.}
\vspace{-0.3cm}
\label{tab:supp_class_iid_50}
\end{center}
\end{table}

==> tables/supp_dataset_size.tex <==
\begin{table}[t]
\centering
{\renewcommand\arraystretch{1.1}
\setlength{\tabcolsep}{1.5mm}{

\begin{tabular}{lcc}
    \toprule
    Methods & ResNet-50 & ViT-S  \\
    \midrule
    ImageNet-50 &   86.60 & 84.72 \\
    ImageNet-50 + \OursCls 1500 & 88.16 & 87.12  \\
    ImageNet-50 + \OursCls 2000 & 88.72 & 88.28 \\
    \cellcolor{mygray-bg}{ImageNet-50 + \OursCls 2500} & \cellcolor{mygray-bg}{\textbf{89.28}} & \cellcolor{mygray-bg}{\textbf{89.36}}  \\ 
    \bottomrule
\end{tabular}}}
\vspace{0.3cm}
\caption{Comparison of the effects of different dataset sizes when \OursCls contains 1500, 2000, and 2500 synthetic images per class, respectively. We evaluate Top-1 accuracy of image classification on ImageNet-50 for ResNet-50 and ViT-S. Experiments show that only using \OursCls with 1500 per class can already improve the accuracy a lot, and using more data can further improve the classification performance of all the models.}
\vspace{-0.3cm}
\label{tab:supp-dataset-size}
\end{table}


==> tables/supp_simple.tex <==
\begin{table}[t]
\centering
{\renewcommand\arraystretch{1.1}
\setlength{\tabcolsep}{1.5mm}{

\begin{tabular}{lcc}
    \toprule
    Methods & ResNet-50 & ViT-S \\
    \midrule
    ImageNet-50 &   86.60 & 84.72 \\
    ImageNet-50 + 3D-DST wo LLM prompts & 88.96 & 88.72 \\
     & {\small \textcolor{ablation_green}{($\uparrow$2.36)}}&  {\small \textcolor{ablation_green}{($\uparrow$4.00)}}\\
    \cellcolor{mygray-bg}{ImageNet-50 + \OursCls (ours)} & \cellcolor{mygray-bg}{\textbf{89.28}} & \cellcolor{mygray-bg}{\textbf{89.36}}  \\\cellcolor{mygray-bg}{}
    & \cellcolor{mygray-bg}{{\small \textcolor{ablation_green}{($\uparrow$2.68)}}} & \cellcolor{mygray-bg}{{\small \textcolor{ablation_green}{($\uparrow$4.64)}}} \\
    \\[-14pt]
    \bottomrule
\end{tabular}}}
\vspace{0.3cm}
\caption{Top-1 accuracy of image classification on ImageNet-50. We evaluate representative models, ResNet-50 and ViT-S. We compare the performances when models are (1) trained purely on ImageNet-50, (2) pretrained on 3D-DST data generated without using LLM prompts (only use simple prompts like class names and keywords from the CAD model descriptions), and then finetuned on ImageNet, (3) pretrained on 3D-DST data, and finetuned on ImageNet-50. Experiments show that our 3D-DST data can help boost the classification accuracy of all the models by a large margin, and using LLM prompts can help achieve better results.}
\vspace{-0.3cm}
\label{tab:supp-simple}
\end{table}
